Evaluating Local Explanations using White-box Models

Evaluating explanation techniques using human subjects is costly, time-consuming and can lead to subjectivity in the assessments. To evaluate the accuracy of local explanations, we require access to the true feature importance scores for a given instance. However, the prediction function of a model usually does not decompose into linear additive terms that indicate how much a feature contributes to the output. In this work, we suggest to instead focus on the log odds ratio (LOR) of the prediction function, which naturally decomposes into additive terms for logistic regression and naive Bayes. We demonstrate how we can benchmark different explanation techniques in terms of their similarity to the LOR scores based on our proposed approach. In the experiments, we compare prominent local explanation techniques and find that the performance of the techniques can depend on the underlying model, the dataset, which data point is explained, the normalization of the data and the similarity metric.

==> inputs/related.tex <==

\section{Related Work}
\label{sec:related_works}

In this section we discuss several ablation and robustness techniques that have been proposed to evaluate the quality of explanations. 

Ablation techniques measure how the black box model reacts to changes in feature values that were deemed important by the explanation. Ablation techniques \citep{hooker2018benchmark} are different variations of the Occlusion Sensitivity method in \cite{zeiler2014visualizing}. In the paper, authors performed occlusion on pixels from different regions of an image. The approach was used to measure the sensitivity of a neural network model after pixels were occluded in each individual image. Most techniques differ in how they change these feature values \citep{fong2017interpretable}. In \citep{hooker2018benchmark}, RemOve And Retrain (ROAR) is proposed to evaluate different explanations techniques based on saliency maps. The black-box model is retrained on an the auxiliary dataset that is striped of pixels deemed important by the explanations. The accuracy of the explanations are calculated as the difference between the predicted class probabilities of the original and the auxiliary instance. Methods such as ROAR are computationally exhaustive as the underlying model needs to be retrained on a large auxiliary data set. Another limitation of this evaluation method is that the new auxiliary data and retrained black-box model deviate from the original data and model and can inhibit new structures and properties. 
%Instead of setting features to a baseline value, authors in \cite{hsieh2021evaluations} propose adversarial perturbations of the input to measure explanation accuracy.  

Robustness of explanations is usually measured by how much the explanation changes when Lipschitz noise  is added to the explained instance.
\cite{alvarez2018robustness} empirically show that some explanation techniques including LIME are not robust to Lipschitz noise and therefore have low robustness. In \citep{camburu2019can}, the robustness of LIME, SHAP and Learn To eXplain (L2X) (\citep{chen2018learning}) are studied following the introduction of irrelevant features to the explained instance in a sentiment analysis task. According to the results, L2X explanations outperform other explanation techniques across different measures of robustness that are proposed in the study. One limitation of this category of evaluation techniques is that changes in feature values of instances can turn them into out-of-distribution data points. As a result, predictions by the black-box model can have high uncertainty as discussed in \citet{ lakkaraju2020robust, rahnama2019study}.

In contrast to these measures, our approach is not based on the idea that measuring the sensitivity of the black-box model is directly correlated with explanation quality. We postulate that to measure explanation quality, we require some kind of true importance score to compare explanations to. For this, we therefore introduce true importance scores of LOR of white-box models.

==> inputs/table_graveyard.tex <==

\begin{table}[htb]
\caption{Mean Spearman's rank correlation between the local baseline and local additive explanations for LIME and SHAP explanations when explaining Naive Bayes Model}
  \centering
\label{table:lime_shap_nbayes_standard}
\begin{tabular}{lrr}
    \toprule
    Data set &   LIME &   SHAP \\
    \midrule
     Attrition                          &  0.0727695 & 0.0564431 & \\
     Breast Cancer                      & -0.192355  & 0.381653 & \\
     Pima Indians                       & -0.0861905 & 0.765841 & \\
     Banknote                           &  0.004     & 0.776    & \\
     Iris                               & -0.008     & 0.464    & \\
     Haberman                           & -0.5       & 0.233766 & \\
     Spambase                           &  0.0349552 & 0.140946 & \\
     Adult                              &  0.906783  & 0.640672 & \\
     Heart Disease                      &  0.897195  & 0.675157 & \\
     Churn                              &  0.848364  & 0.801399 & \\
     Hattrick                           &  0.773209  & 0.748734 & \\
     HR                                 &  0.90979   & 0.498115 & \\
     Insurance                          &  0.731152  & 0.33468  & \\
     Audit                              &  0.0496609 & 0.249443 & \\
     Loan                               &  0.200549  & 0.0324037 & \\
     Donors                             &  0.201683  & 0.0849539 &\\
     Seismic                            &  0.805699  & 0.300376  & \\
     Thera                              &  0.215245  & 0.0336269 & \\
     Banking                            &  0.75175   & 0.305849  & \\
     Titanic                            &  0.830476  & 0.395048  & \\
     
        
      \midrule
    Average             &  0.372337  & 0.395955  \\
 Standard Deviation  &  0.439834  & 0.258113  \\
    \hline

 \bottomrule
\end{tabular}
\end{table}




\begin{table}[htb]
\caption{Mean Spearman's rank correlation for explanations between the local baseline and explanations of Logistic Regression}
\label{table:lime_shap_lreg_standard}
  \centering
\begin{tabular}{lrr}
    \toprule
    Data set &   LIME &   SHAP \\
    \midrule
     Attrition                          &  0.643567  & 0.243841 \\
     Breast Cancer                      & -0.123764  & 0.912763 \\
     Pima Indians                       & -0.0857143 & 0.942317 \\
     Banknote                           &  0.04      & 0.952    \\
     Iris                               & -0.064     & 0.808    \\
     Haberman                           & -0.220779  & 0.649351 \\
     Spambase                           & -0.594526  & 0.402385 \\
     Adult                              &  0.693911  & 0.470788 \\
     Heart Disease                      &  0.42355   & 0.593762 \\
     Churn                              &  0.720874  & 0.643877 \\
     Hattrick                           &  0.590986  & 0.737762 \\
     HR                                 &  0.446307  & 0.404132 \\
     Insurance                          &  0.682999  & 0.138279 \\
     Audit                              &  0.642483  & 0.511469 \\
     Loan                               &  0.594592  & 0.603591 \\
     Donors                             &  0.193084  & 0.29035  \\
     Seismic                            &  0.738776  & 0.530586 \\
     Thera                              &  0.797695  & 0.612586 \\
     Banking                            &  0.470248  & 0.575738 \\
     Titanic                            &  0.595358  & 0.19925  \\
      \midrule
     Average           &  0.359282  & 0.561141 \\
    Standard Deviation &  0.388579  & 0.232314 \\
    \hline

 \bottomrule
\end{tabular}
\end{table}





\begin{table}[t]
\caption{Mean Spearman's rank correlation for LPI explanations between the local baseline and local non-additive explanations of Naive Bayes Model}
  \centering
\label{table:lpi_standard}
\begin{tabular}{lrr}
    \toprule
    Data set &  LR &  Naive Bayes  \\
    \midrule
     Attrition          &              0.589034 &                0.297069 \\
     Breast Cancer      &              0.914136 &                0.52985  \\
     Pima Indians       &              0.872857 &                0.83     \\
     Banknote           &              0.788    &                0.9      \\
     Iris               &              0.912    &                0.587935 \\
     Haberman           &              0.62987  &                0.922078 \\
     Spambase           &              0.775727 &                0.638742 \\
     Adult              &              0.64276  &                0.866461 \\
     Heart Disease      &              0.550689 &                0.855697 \\
     Churn              &              0.534122 &                0.829333 \\
     Hattrick           &              0.653    &                0.667857 \\
     HR                 &              0.530753 &                0.856923 \\
     Insurance          &              0.707853 &                0.725212 \\
     Audit              &              0.836725 &                0.404748 \\
     Loan               &              0.535683 &                0.46291  \\
     Donors             &              0.593438 &                0.610011 \\
     Seismic            &              0.591856 &                0.8187   \\
     Thera              &              0.747881 &                0.480384 \\
     Banking            &              0.386409 &                0.815246 \\
     Titanic            &              0.621316 &                0.874048 \\
      \midrule
    Average            &              0.646597 &                0.675199 \\
    Standard Deviation &              0.177592 &                0.209359 \\
    \hline
 \bottomrule
\end{tabular}
\end{table}



\begin{table}[t]
\caption{Average rank of explanation techniques based on the mean rank correlation across all data sets}
\label{table:rank_odds_standardized}
\begin{center}
\begin{tabular}{ccc}
    Model & Technique & Average Rank \\
    \hline
    \multirow{ 3}{*}{Logistic Regression}    & LIME & 2.2\\
        & SHAP & 2.05\\
        & LPI & \textbf{1.75} \\
     \midrule
     \multirow{ 3}{*}{Naive Bayes}    & LIME &  2.05 \\
        & SHAP & 2.6 \\
        & LPI & \textbf{1.35} \\
    \bottomrule
\end{tabular}
\end{center}
\label{tab:multicol}
\end{table}


\begin{table}[t]
  \caption{The average rank of explanation techniques based on mean Spearman's rank correlation across all datasets for each pre-processing transformation when explaining the na\"ive Bayes Model}
  \label{table:final_rank_preprocessing_nbayes}
  \centering
    \begin{tabular}{lrrr}
    \toprule
            %& \multicolumn{3}{c}{na\"ive Bayes} \\
    %\toprule
               &   LIME &   SHAP &   LPI \\
        \midrule
         Standard & 0.372 & 0.396 & \textbf{0.699} \\
         Robust   & 0.386 & 0.397 & \textbf{0.699} \\
         Minmax   & 0.401 & 0.396 & \textbf{0.697} \\
    \bottomrule
    \end{tabular}
\end{table}


\begin{table}[t]
  \caption{The average rank of explanation techniques based on mean Spearman's rank correlation across all datasets for each pre-processing transformation when explaining the Logistic Regression Model}
  \label{table:final_rank_preprocessing_lreg}
  \centering
    \begin{tabular}{lrrr}
    \toprule
           % & \multicolumn{3}{c}{Logistic Regression} \\
   % \toprule
               &   LIME &   SHAP &   LPI  \\
        \midrule
         Standard & 0.359 & 0.561 & \textbf{0.671} \\
         Robust   & 0.344 & \textbf{0.714} & 0.433 \\
         Minmax   & \textbf{0.398} & 0.223 & 0.093 \\
    \bottomrule
    \end{tabular}
\end{table}






\begin{table*}[htb]
\caption{Average Spearman's rank correlation between the true importance scores and local explanations for LIME, SHAP and LPI explanations when explaining Logistic Regression and na\"ive Bayes Models}
  \centering
  \small{
\label{table:lime_shap_lpi}
\begin{tabular}{l|ccc|cccl|ccc|ccc}
    \toprule
     Model &  \multicolumn{3}{c}{Logistic Regression} &  \multicolumn{3}{|c}{Na\"ive Bayes}   & &\multicolumn{3}{c}{Logistic Regression} &  \multicolumn{3}{|c}{Na\"ive Bayes}  \\ \hline
    dataset &   LIME &   SHAP & LPI &   LIME &   SHAP & LPI & dataset &   LIME &   SHAP & LPI &   LIME &   SHAP & LPI \\ \hline
      Adult              &  0.694 & 0.471 & 0.643 &  0.907 & 0.641 & 0.866 &  Hattrick           &  0.591 & 0.738 & 0.653 &  0.773 & 0.749 & 0.668 \\

     Attrition          &  0.644 & 0.244 & 0.589 &  0.073 & 0.056 & 0.297 &  Heart D.     &  0.424 & 0.594 & 0.551 &  0.897 & 0.675 & 0.856 \\

     Audit              &  0.642 & 0.511 & 0.837 &  0.05  & 0.249 & 0.405 &  Insurance          &  0.683 & 0.138 & 0.708 &  0.731 & 0.335 & 0.725 \\

     Banking            &  0.47  & 0.576 & 0.386 &  0.752 & 0.306 & 0.815 &  Iris               & -0.064 & 0.808 & 0.912 & -0.008 & 0.464 & 0.588 \\

     Banknote           &  0.04  & 0.952 & 0.788 &  0.004 & 0.776 & 0.9   &   Loan               &  0.595 & 0.604 & 0.536 &  0.201 & 0.032 & 0.463 \\

     Breast C.      & -0.124 & 0.913 & 0.914 & -0.192 & 0.382 & 0.53   &  Pima I.       & -0.086 & 0.942 & 0.873 & -0.086 & 0.766 & 0.83  \\
     Churn              &  0.721 & 0.644 & 0.534 &  0.848 & 0.801 & 0.829 &  Seismic            &  0.739 & 0.531 & 0.592 &  0.806 & 0.3   & 0.819 \\

     Donors             &  0.193 & 0.29  & 0.593 &  0.202 & 0.085 & 0.61  &  Spambase           & -0.595 & 0.402 & 0.776 &  0.035 & 0.141 & 0.639 \\

     HR                 &  0.446 & 0.404 & 0.531 &  0.91  & 0.498 & 0.857   &  Thera              &  0.798 & 0.613 & 0.748 &  0.215 & 0.034 & 0.48  \\
     Haberman           & -0.221 & 0.649 & 0.63  & -0.5   & 0.234 & 0.922   &  Titanic            &  0.595 & 0.199 & 0.621 &  0.83  & 0.395 & 0.874 \\

    
    \hline
      \midrule
        Average            &  0.359 & 0.561 & 0.671 &  0.372 & 0.396 & 0.699 \\
     Stand. Deb. &  0.389 & 0.232 & 0.14  &  0.44  & 0.258 & 0.183 \\
 \bottomrule
\end{tabular}
}
\end{table*}
